Augmentation by Counterfactual Explanation -- Fixing an Overconfident Classifier

A highly accurate but overconfident model is ill-suited for deployment in critical applications such as healthcare and autonomous driving. The classification outcome should reflect a high uncertainty on ambiguous in-distribution samples that lie close to the decision boundary. The model should also refrain from making overconfident decisions on samples that lie far outside its training distribution, far-out-of-distribution (far-OOD), or on unseen samples from novel classes that lie near its training distribution (near-OOD). This paper proposes an application of counterfactual explanations in fixing an over-confident classifier. Specifically, we propose to fine-tune a given pre-trained classifier using augmentations from a counterfactual explainer (ACE) to fix its uncertainty characteristics while retaining its predictive performance. We perform extensive experiments with detecting far-OOD, near-OOD, and ambiguous samples. Our empirical results show that the revised model have improved uncertainty measures, and its performance is competitive to the state-of-the-art methods.

==> other/original_eccv.tex <==
% \documentclass[10pt,twocolumn,letterpaper]{article}

% \usepackage{wacv}
% \usepackage{times}
% \usepackage{epsfig}
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{booktabs}
% % Include other packages here, before hyperref.



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %
% %%% IMPORTANT - These next three lines are CRUCIAL.
% %               (1) PLEASE enter your paper ID (given by CMT) replacing the
% %                   '****' right below here with the ID from CMT.
% %               (2) If you are submitting to the Algorithms track, then uncomment
% %                   the \wacvalgorithmstrack line below. If you are submitting to the
% %                   Applications track, then uncomment the \wacvapplicationstrack line.
% %                   If you do not update this properly, we cannot guarantee
% %                   that your paper will be evaluated according to the correct
% %                   review criteria!
% %               (3) Leave the \wacvfinalcopy commented out for the submission
% %                   version, but UNCOMMENT it for your CAMERA-READY upload.
 
% %(1)
% \def\wacvPaperID{****} % Enter the WACV Paper ID here

% %(2)
% %\wacvalgorithmstrack   % Uncomment this line if you are submitting to the Algorithms Track.
% \wacvapplicationstrack % Uncomment this line if you are submitting to the Applications Track.

% %(3)
% %\wacvfinalcopy % *** Uncomment this line for the final submission


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




% % If you comment hyperref and then uncomment it, you should delete
% % egpaper.aux before re-running latex.  (Or just hit 'q' on the first latex
% % run, let it finish, and you should be clear).
% \ifwacvfinal
% \usepackage[breaklinks=true,bookmarks=false]{hyperref}
% \else
% \usepackage[pagebackref=true,breaklinks=true,colorlinks,bookmarks=false]{hyperref}
% \fi

% % Pages are numbered in submission mode, and unnumbered in camera-ready
% \pagestyle{empty}

% \def\httilde{\mbox{\tt\raisebox{-.5ex}{\symbol{126}}}}

% \begin{document}

% %%%%%%%%% TITLE
% \title{Augmentation by Counterfactual Explanation - \\
% Fixing an Overconfident Classifier}

% \author{First Author\\
% Institution1\\
% Institution1 address\\
% {\tt\small firstauthor@i1.org}
% % For a paper whose authors are all at the same institution,
% % omit the following lines up until the closing ``}''.
% % Additional authors and addresses can be added with ``\and'',
% % just like the second author.
% % To save space, use either the email address or home page, not both
% \and
% Second Author\\
% Institution2\\
% First line of institution2 address\\
% {\tt\small secondauthor@i2.org}
% }

% \maketitle
% \thispagestyle{empty}

% %%%%%%%%% ABSTRACT
% \begin{abstract}
% A highly accurate but overconfident model is ill-suited for decision-making pipelines, especially in critical applications such as healthcare and autonomous driving. The classification outcome should reflect a high uncertainty on ambiguous in-distribution samples that lie close to the decision boundary. The model should also refrain from making overconfident decisions on samples that lie far outside its training distribution, far-out-of-distribution (far-OOD), or on  unseen samples from novel classes that lie near its training distribution (near-OOD). This paper proposes a method to fine-tune a given pre-trained classifier to fix its uncertainty characteristics while retaining its predictive performance.


% We propose using a Progressive Counterfactual Explainer (PCE) to generate counterfactually augmented data (CAD) for fine-tuning the classifier. The PCE is a form of conditional Generative Adversarial Networks (cGANs) trained to generate samples that visually traverse the separating boundary of the classifier. The discriminator of the PCE serves as a density estimator to identify and reject OOD samples. We perform extensive experiments with detecting far-OOD, near-OOD, and ambiguous samples. Our empirical results show that our model improves the uncertainty of the baseline, and its performance is competitive to other methods that require a significant change or a complete re-training of the baseline model.
% % \keywords{OOD Detection, Uncertainty, GAN, Data Augmentation}
% \end{abstract}

% %%%%%%%%% BODY TEXT
% \section{Introduction}

% \newcommand{\blue}[1]{\textcolor[RGB]{0, 0, 255}{#1}}
% \newcommand{\nood}[1]{\textcolor[RGB]{196, 78, 82}{#1}}

% \newcommand{\aid}[1]{\textcolor[RGB]{34,135, 60}{#1}}

% \newcommand{\uid}[1]{\textcolor[RGB]{76,114, 176}{#1}}

% \newcommand{\food}[1]{\textcolor[RGB]{221, 132, 82}{#1}}
% Deep neural networks (DNN) are increasingly being used in \emph{decision-making} pipelines for real-world high-stake applications such as medical diagnostics~\cite{esteva2017dermatologist} and autonomous driving~\cite{Autonomous}. For optimal decision making, the DNN should produce accurate predictions as well as quantify uncertainty over its predictions~\cite{Gal2016UncertaintyID,christian2017}. While substantial efforts are made to engineer highly accurate architectures~\cite{huang2017densely}, many existing state-of-the-art DNNs do not capture the uncertainty correctly~\cite{pmlr-v48-gal16}. This hinders the re-use of openly available pre-trained models for real-world applications. We proposed to fine-tune the given \emph{pre-trained} DNN on counterfactually augmented data, to improve its uncertainty quantification  while retaining its original predictive accuracy. 





% %Any classification model is essentially learning a hyperplane to separate samples from different classes. 
% Accuracy only captures the proportion of samples that are on the correct side of the decision boundary. However, it ignores the relative distance of the sample from the decision boundary~\cite{krishnan2020improving}. Ideally, samples closer to the boundary should have high uncertainty. The actual predicted value from the classifier should reflect this uncertainty via a low confidence score~\cite{Hllermeier2021AleatoricAE}. Conventionally, DNNs are trained on hard-label datasets to minimize a negative log-likelihood (NLL) loss.  Such models tend to over-saturate on NLL and end-up learning very sharp decision boundaries~\cite{guo2017calibration,mukhoti2020calibrating}. The resulting classifiers extrapolate over-confidently on ambiguous, near boundary samples, and the problem amplifies as we move to OOD regions~\cite{Gal2016UncertaintyID}.


% \begin{figure*}[htbp]
%   \centering
%   \includegraphics[width=1.0\linewidth]{figures/results_all.pdf}
%   \caption{   \footnotesize Comparison of the uncertainty estimates from the baseline, before and after fine-tuning with ACE. Each row represents a different dataset. A) Fine-tuning has little effect on the predicted entropy (PE) of \textbf{\uid{in-distribution (iD)}} samples. We use PE to identify \textbf{\aid{ambiguous iD (AiD)}} samples (B) and \textbf{\nood{near-OOD}} samples (C). D-E) We use the discriminator of the PCE to identify \textbf{\food{far-OOD}} samples (last two columns). The legend shows the AUC-ROC for binary classification over uncertain samples and iD samples. Our method improved the uncertainty estimates across the spectrum.  }
%   \label{fig:all}
% \end{figure*}

% We consider two types of uncertainty: \emph{epistemic uncertainty}, caused due to limited data and knowledge of the model, and \emph{aleatoric uncertainty}, caused by inherent noise or ambiguity in the data~\cite{KIUREGHIAN2009105}.  We evaluate these uncertainties with respect to three test  distributions (\emph{see} Fig~\ref{fig:all}):

% \begin{itemize}
% \item \aid{\bf{Ambiguous in-Distribution (AiD)}}: These are the samples within the training distribution that have an inherent ambiguity in their class labels. Such ambiguity represents high aleatoric uncertainty arising from class overlap or noise~\cite{smith2018understanding}, \eg an image of a `5' that is similar to a `6'.

% \item \nood{\bf{Near-OOD}}: Near-OOD represents a label shift where label
% space is different between ID and OOD data.  It has high epistemic uncertainty arising from the classifier's limited information on unseen data. We use samples from unseen classes of the training distribution as near-OOD. 


% \item \food{\bf{Far-OOD}}: Far-OOD represents data distribution that is significantly different from the training distribution. It has high epistemic uncertainty arising from mismatch between different data distributions.

% \end{itemize}

% Much of the earlier work focuses on threshold-based detectors that use information from a pre-trained DNN to identify OOD samples~\cite{temperature_scaling,hendrycks17baseline,huang2021on,wang2021can,9156473}. Such methods predominantly focus on far-OOD detection and often do not address the over-confidence problem in DNN. In another line of
% research, variants of Bayesian models~\cite{neal2012bayesian,pmlr-v48-gal16} and ensemble learning~\cite{Snapshot,NIPS2017_9ef2ed4b} were explored to provide reliable uncertainty estimates. Recently, there is a shift towards designing generalizable DNN that provide robust uncertainty estimates in a single forward pass~\cite{van2021feature,chen2021atom,mukhoti2021deterministic}. Such methods usually propose changes to the DNN architecture~\cite{sun2021react}, training procedure~\cite{zhang2017mixup} or loss functions~\cite{Mukhoti2020CalibratingDN} to encourage separation between ID and OOD data. Popular methods include, training deterministic DNN with a distance-aware feature space~\cite{van2020uncertainty,Liu2020SimpleAP} and 
% regularizing DNN training with a generative model that simulates OOD data~\cite{lee2018training}. However, these methods require a DNN model to be trained from scratch and are not compatible with an existing pre-trained DNN. Also, they may use auxiliary data to learn to distinguish OOD inputs~\cite{liu2020energy}.







% %The principled approach for UQ relies on Bayesian methods (BNN) that model the network weights and activations in a probabilistic framework \cite{blundell2015weight,neal2012bayesian}. However BNNs are computationally expensive to train~\cite{kendall2017uncertainties} and arguably sub-optimal in predictive accuracy~\cite{pmlr-v37-hernandez-lobatoc15}.Many methods have been proposed to approximate Bayesian inference, such as MC Dropout \cite{pmlr-v48-gal16} and Deep Ensembles \cite{NIPS2017_9ef2ed4b,Wen2020BatchEnsembleAA}. However, these methods require training the DNN from scratch and hence, cannot be used with a given pre-trained DNN.

% %Consequently, there is a surge of interest in estimating uncertainty in a deterministic DNN  using a single forward pass, with fast test-time inference. Recent work focuses on training DL models with a distance-aware feature space\cite{van2020uncertainty,Liu2020SimpleAP} and combining them with feature-density based estimators\cite{van2021improving}. However, these approaches require changes to the DNN architecture and the network is trained from scratch with added constraints.  Hence, they cannot be applied to a pre-trained DNN. Our method aims to improve uncertainty estimates from an existing pre-trained DNN.


% In this work, we introduce an augmentation by counterfactual explanation (ACE) strategy to fine-tune an existing \emph{pre-trained} DNN. Fine-tuning improves the uncertainty estimates without changing the network's architecture or compromising on its predictive performance. ACE uses a progressive counterfactual explainer (PCE) similar to Lang \etal~\cite{explaining_in_style} and Singla \etal~\cite{singla2019explanation,singla2021explaining} to generate counterfactually augmented data (CAD). The discriminator of the PCE is a density estimator and is used in a threshold-based selection function to identify and reject far-OOD samples.

% The PCE is a conditional-Generative Adversarial Network (cGAN)-based explanation function that explains the decision of a DNN by gradually perturbing a query image to flip its classification decision. We used PCE to generate augmented samples closer to the decision boundary. We assign soft labels to these generated samples that mimic their distance from the boundary. Fine-tuning on such augmented data helps the DNN to recover from the over-saturation on NLL loss, thus making the decision boundary smoother. Smooth decision boundary facilitates improved uncertainty estimates for AiD and near-OOD samples and also makes the classifier robust to adversarial attacks.


% %We introduce a new data augmentation strategy, Augmentation by Counterfactual Explanation (ACE), that improves the UQ of a \emph{pre-trained} DNN while retaining its predictive accuracy. Specifically, we learn a progressive counterfactual explainer (PCE) to derive explanations for the given \emph{pre-trained} DNN. The PCE is a Generative Adversarial Network (GAN)-based explainer that generates gradual perturbations of a query image such that the classification decision changes from the original to a counterfactual class. We used the GAN-based PCE to derive data augmentation (DA) in the regions closer to the decision boundary and associate soft labels with the generated samples that mimic their distance from the decision boundary. Our experiments show that retraining the given DNN on such DA improves its uncertainty estimates for AiD and nearby OOD samples. Previously, Mukhoti \etal~\cite{mukhoti2021deterministic} have shown that a single output layer DNN cannot capture both epistemic and aleatoric uncertainty together. Hence, we use the data likelihood estimates from the discriminator of the PCE as a selection function that abstains the improved DNN from making predictions on far-away OOD samples.




% %assume we are given a pre-trained black box, with a good accuracy but sub-optimal uncertainty characteristics. Our goal is to achieve an improvement in uncertainty estimation on out-of-distribution (OOD) and ambiguous in-distribution (AiD) samples, without significantly affecting the accuracy. More specifically, we consider:



%  %is a challenging problem as there is no ground truth available for uncertainty estimates.
% %mkes overconfident predictions on out-of-distribution (OOD) and ambiguous in-distribution (iD) samples.





% %Fig.\ref{fig:1} (first column) shows the two moons 2D dataset. Top row shows a classifier trained on data with overlapping classes. The bottom row shows a classifier trained on non-overlapping classes with nearby OOD (red) and far-away OOD (black) test samples. Fig.\ref{fig:1}.a shows the confidence distribution of the given DNN. It is uncertain only in a thin region along the decision boundary, and makes over-confident predictions on AiD and nearby OOD samples. Our proposed ACE strategy improved the predicted confidence over all three test samples, as shown in Fig.\ref{fig:1}.


% %Our strategy is to train a conditional explainer to generate augmented samples and perform fine-tuning. The explainer follows the idea of counterfactual explainer in~[??,??] and serves two goals: (1) It generates synthetic samples close to the decision boundary of the DNN, thereby reducing the over-sharpness (or over-confidence) of the classifier. (2) The counterfactual explainer is equipped with a discriminator that can fix the OOD issue by abstaining from making a decision.

% %Our method requires minimal hyper-parameter tuning and can be used to improve uncertainty estimates of any \emph{off-the-shelf} DNN, without compromising on predictive accuracy. 

% Our contributions are as follows: (1)
% We propose a novel strategy to fine-tune an existing \textit{pre-trained} DNN to improve its uncertainty estimates and facilitate its deployment in real-world applications. (2) Our approach generates counterfactual augmentations near the decision boundary, allowing the classifier to widen its boundary, to successfully capture the uncertainty over ambiguous-iD and near-OOD samples. (3) Our GAN-based augmenter provides a density estimator (the discriminator) to detect far-OOD samples.

% We provide a comprehensive evaluation of our method on specifically defined test datasets to capture different uncertainties. Furthermore, our fine-tuned classifier exhibits better robustness to popular adversarial attacks.



% %------------------------------------------------------------------------
% \section{Method}





% In this paper, we consider a pre-trained DNN classifier, $f_{\theta}$, with good prediction accuracy but sub-optimal uncertainty estimates. We assume $f_{\theta}$ is a differentiable function and we have access to its gradient with respect to the input, $\nabla_\mathbf{x}f_{\theta}(\mathbf{x})$, and to its final prediction outcome $f_{\theta}(\mathbf{x})$.  We also assume access to either the training data for $f_{\theta}$, or an equivalent dataset with competitive prediction accuracy. 
% We further assume that the training dataset for $f_{\theta}$ has hard labels $\{0,1\}$ for all the classes. 

% Our goal is to \emph{fine-tune} $f_{\theta}$ such that the revised model provides better uncertainty estimates, while retaining its original predictive accuracy. 
% %More specifically, we aim to improve uncertainty estimates for OOD and ambiguous samples. 
% We use a progressive counterfactual explainer (PCE) to generate counterfactually augmented data. This data is then used to apply a few updates to $f_{\theta}$, to gradually widen its decision boundary, resulting in improved uncertainty estimates on ambiguous and near-OOD samples. The PCE generates realistic perturbations of a given query image while gradually traversing the decision boundary between the classes, as defined by $f_{\theta}$\cite{singla2019explanation,explaining_in_style}. We used the PCE with a conditional-GAN backbone that is trained with respect to $f_{\theta}$. The discriminator of the cGAN-based PCE models is a density estimator that provides essential information to enhance  $f_{\theta}$ far-OOD detection. More specifically, we used the discriminator as a \emph{selection function} to abstain $f_{\theta}$ from making prediction on far-OOD samples. Fig.~\ref{fig:2} summarizes our approach. 




% The remaining sections are structured as follow: we first formulate the cGAN-based PCE model in Section~\ref{sec:AN}. In Section~\ref{sec:ACE}, we describe our novel Augmentation by Counterfactual Explanation (ACE) strategy that uses the trained PCE to generate CDA and fine-tune $f_{\theta}$. Finally, in Section~\ref{sec:SC}, we combine the discriminator from the PCE with the fine-tuned $f_{\theta}$ to provide our final classifier.

% \paragraph{Notation:} The classification function is defined as $f_{\theta}: \mathbb{R}^d \rightarrow \mathbb{R}^K$, where $\theta$ represents model parameters. The training dataset for $f_{\theta}$ is defined as $\mathcal{D} = \{\mathcal{X}, \mathcal{Y}\}$, where $\mathbf{x} \in \mathcal{X} $ represents an input space and  $y \in \mathcal{Y} = \{1,2, \cdots, K\}$ is a label set over $K$ classes.  The classifier produces point estimates to approximate the posterior probability $\mathbb{P}(y|\mathbf{x}, \mathcal{D})$. 

% %We use $\max_{k}f_{\theta}(\mathbf{x})$, $\argmaxD_{k}f_{\theta}(\mathbf{x})$ and $-\sum[f_{\theta}(\mathbf{x})]_k \log[f_{\theta}(\mathbf{x})]_k$ to define confidence, predicted class and predictive entropy, respectively.
 
 
% \begin{figure*}[htbp]
%   \centering
%   \includegraphics[width=1.0\linewidth]{figures/Schematic.pdf}
%   \footnotesize
%   \caption{(a) Given a \emph{pre-trained} classifier $f_{\theta}$, we learn a c-GAN based progressive counterfactual explainer (PCE) $G(\mathbf{x}, \mathbf{c})$, while keeping $f_{\theta}$ fixed. (b) The trained PCE creates counterfactually augmented data. (c) A combination of original training data and augmented data is used to fine-tune the classifier, $f_{\theta + \Delta}$. (d) The discriminator from PCE serves as a selection function to detect and reject OOD data.   }
%   \label{fig:2}
% \end{figure*} 

  
% \subsection{Progressive Counterfactual Explainer (PCE) }
% \label{sec:AN}
%  We designed the PCE network to take a query image ($\mathbf{x} \in \mathbb{R}^d$) and a desired classification outcome ($\mathbf{c} \in \mathbb{R}^K$) as input, and create a perturbation of a query image ($\hat{\mathbf{x}}$) such that $f_{\theta}(\hat{\mathbf{x}}) \approx \mathbf{c}$. Our formulation, $\hat{\mathbf{x}}= G(\mathbf{x}, \mathbf{c})$ allows us to use $\mathbf{c}$ to traverse through the decision boundary of $f_{\theta}$ from the original class to a counterfactual class. Following previous work~\cite{explaining_in_style,singla2019explanation,singla2021explaining}, we design the PCE to satisfy the following three properties:
 
%  \begin{enumerate}
%      \item \textbf{Data consistency: } The perturbed image, $\hat{\mathbf{x}}$ should be realistic and should resemble samples in $\mathcal{X}$.
%      \item \textbf{Classifier consistency:} The perturbed image, $\hat{\mathbf{x}}$ should produce
% the desired output from the classifier $f_{\theta}$ \ie $f_{\theta}(G(\mathbf{x}, \mathbf{c})) \approx \mathbf{c}$.

% \item  \textbf{Self consistency:} Using the original classification decision $f_{\theta}(\mathbf{x})$ as condition, the PCE should produce a perturbation that is very similar to the query image, \ie $G(G(\mathbf{x}, \mathbf{c}), f_{\theta}(\mathbf{x})) = \mathbf{x}$ and $G(\mathbf{x}, f_{\theta}(\mathbf{x})) = \mathbf{x}$.
%  \end{enumerate}
%  \emph{Data Consistency:} 
%  We formulate the PCE as a cGAN that learns the underlying data distribution of the input space $\mathcal{X}$ without an explicit likelihood assumption. The GAN model comprised of two networks -- the generator $G(\cdot)$ and the discriminator $D(\cdot)$. The $G(\cdot)$ learns to generate fake data, while the $D(\cdot)$  is trained to distinguish between the real and fake samples.  We jointly train $G, D$ to optimize the following logistic adversarial loss~\cite{goodfellow2014generative},
% \begin{equation}
% \begin{split}
%     \mathcal{L}_{\text{adv}}(D,G) = \mathbb{E}_{\mathbf{x}}[\log D(\mathbf{x}) + \log (1 - D(G(\mathbf{x}, \mathbf{c})))]
% \end{split}
% \end{equation}
 
%  Our architecture for the cGAN is adapted from StyleGANv2~\cite{abdal2019image2stylegan}. We formulate the generator as $G(\mathbf{x}, \mathbf{c}) = g(e(\mathbf{x}), \mathbf{c})$, a composite of two functions, an image encoder $e(\cdot)$ and a conditional decoder $g(\cdot)$~\cite{abdal2019image2stylegan}. The encoder function $e: \mathcal{X} \rightarrow \mathcal{W}^+$, learns a mapping from the input space $\mathcal{X}$ to an extended latent space $\mathcal{W}^+$. The  $\mathcal{W}^+$ represents a concatenation of $L$ different latent representations ($w_l$), one for each layer of the decoder $g(\cdot)$. The conditional decoder $g(\cdot)$, maps the embedding back to the input space $\mathcal{X}$ while respecting the condition $\mathbf{c}$. We provide condition information to the decoder by concatenating the condition $\mathbf{c}$ to each $w_l \in \mathcal{W}^+$. The decoder further transforms the layer-specific latent representation into a layer-specific style-vector as $s_l = A_l([w_l , \phi(\mathbf{c})])$ where, $A_l$ is an affine transformation and $\phi(\mathbf{c})$ is an embedding for $\mathbf{c}$. Further, we also extended the discriminator network $D(\cdot)$ to have auxiliary information from the classifier $f_{\theta}$. Specifically, we concatenate the penultimate activations from the $f_{\theta}(\mathbf{x})$ with the penultimate activations from the $D(\mathbf{x})$, to obtain a revised representation  before the final fully-connected layer of the discriminator.
% The detailed architecture is summarized in supplementary material (SM).
 
%  We also borrow the concept of path-length regularization $\mathcal{L}_{\text{reg}}(G)$ from StyleGANv2 to enforce smoother latent space interpolations for the generator. $\mathcal{L}_{\text{reg}}(G) = \mathbb{E}_{\mathbf{w}\sim e(\mathbf{x}), \mathbf{x}\sim \mathcal{X}} (||J^T_\mathbf{w}\mathbf{x}||_2 - a)^2$, where $\mathbf{x}$ denotes random images from the training data, $J_{\mathbf{w}}$ is the Jacobian matrix, and $a$ is a constant that is set dynamically during optimization. 
% \newline
% \newline
% \emph{Classifier consistency: }By default, GAN training is independent of the classifier $f_{\theta}$. We add a classifier-consistency loss to regularize the generator and ensure that the actual classification outcome for the generated image $\hat{\mathbf{x}}$, is similar to the condition $\mathbf{c}$ used for generation. We enforce classification-consistency by a
% KullbackLeibler (KL) divergence loss as follow\cite{singla2019explanation,singla2021explaining},
% \begin{equation}
%     \mathcal{L}_{f}(G) = D_{KL}(f_{\theta}(\hat{\mathbf{x}})|| \mathbf{c})
% \end{equation}
% \emph{Self consistency: }We define the following reconstruction loss to regularize and constraint the Generator to preserve maximum information between the original image $\mathbf{x}$ and its reconstruction $\bar{\mathbf{x}}$,

% \begin{equation}
%     \mathcal{L}(\mathbf{x}, \bar{\mathbf{x}}) = ||\mathbf{x} - \bar{\mathbf{x}}||_1 + ||e(\mathbf{x}) - e(\bar{\mathbf{x}})||_1 
% \end{equation}

% Here, first term is a distance loss between the input and the reconstructed image, and the second term is a style reconstruction loss adapted from StyleGANv2~\cite{abdal2019image2stylegan}. We minimize the reconstruction loss to satisfy the identify constraint on self reconstruction using $\bar{\mathbf{x}}_{self} = G(\mathbf{x}, f_{\theta}(\mathbf{x}))$. We further insure that the PCE learns a reversible perturbation by recovering the original image from a given perturbed image $\hat{\mathbf{x}}$ as  $\bar{\mathbf{x}}_{\text{cyclic}} = G(\hat{\mathbf{x}}, f_{\theta}(\mathbf{x}))$, where $\hat{\mathbf{x}} = G(\mathbf{x}, \mathbf{c})$ with some condition $\mathbf{c}$. Our final reconstruction loss is defined as,
% \begin{equation}
%     \mathcal{L}_{\text{rec}}(G) = \mathcal{L}(\mathbf{x}, \bar{\mathbf{x}}_{\text{self}}) + \mathcal{L}(\mathbf{x}, \bar{\mathbf{x}}_{\text{cyclic}})
% \end{equation}
% \emph{Objective function: }Finally, we trained our model in an end-to-end fashion to learn parameters for the two networks,  while keeping the classifier $f_{\theta}$ fixed. Our overall objective function is

% \begin{equation}
% \begin{split}
%     \min_{G} \max_{D} \lambda_{\text{adv}}\left( \mathcal{L}_{\text{adv}}(D,G) +     \mathcal{L}_{\text{reg}}(G)\right) \\
%     + \lambda_{f} \mathcal{L}_f(G) + \lambda_{\text{rec}} \mathcal{L}_{\text{rec}}(G),
% \end{split}
% \label{eq:5}
% \end{equation}

% where, $\lambda$'s are the hyper-parameters to balance each of the loss terms.

% \subsection{Augmentation by Counterfactual Explanation}
% \label{sec:ACE}
% Given a query image $\mathbf{x}$, the trained PCE generates a series of  perturbations of $\mathbf{x}$ that gradually traverse the decision boundary of $f_{\theta}$ from the original class to a counterfactual class, while still remaining plausible and realistic-looking. 
% %This series of  perturbations is essentially mimicking a traversal on a latent manifold, as guided by the condition $\mathbf{c}$. Our trained AN enables conditional generation of an image at any point on the manifold as $G(\mathbf{x}, \mathbf{c})$ (\emph{see} Fig.\ref{fig:2}.B). 
% We modify $\mathbf{c}$ to represent different steps in this traversal.  We start from a high data-likelihood region for original class $k$ ($\mathbf{c}[k] \in [0.8, 1.0]$), walk towards the decision hyper-plane ($\mathbf{c}[k] \in [0.5, 0.8)$), and eventually cross the decision boundary ($\mathbf{c}[k] \in [0.2, 0.5)$) to end the traversal in a high data-likelihood region for the counterfactual class $k_c$ ($\mathbf{c}[k] \in [0.0, 0.2)$). Accordingly, we  set $\mathbf{c}[k_{c}] = 1- \mathbf{c}[k]$.  

% Ideally, the predicted confidence from NN should be  indicative of the distance from the decision boundary. Samples that lies close to the decision boundary should have low confidence, and confidence should increase as we move away from the decision boundary. We used $\mathbf{c}$ as a pseudo indicator of confidence to generate synthetic augmentation. Our augmentations are essentially showing how the query image $\mathbf{x}$ should be modified to have low/high confidence. 


% To generate CAD, we randomly sample a subset of real training data as $\mathcal{X}_r {\displaystyle \subset }\mathcal{X}$. Next, for each $\mathbf{x} \in \mathcal{X}_r$ we generate multiple augmentations ($\hat{\mathbf{x}} = G(\mathbf{x}, \mathbf{c})$) by randomly sampling $\mathbf{c}[k] \in [0,1]$. We used $\mathbf{c}$ as soft label for the generate sample while fine-tuning the $f_{\theta}$. The  $\mathcal{X}_{c}$ represents our pool of generated augmentation images. Finally, we create a new dataset by randomly sampling images from $\mathcal{X}$ and $\mathcal{X}_c$. We fine-tune the $f_{\theta}$ on this new dataset, for only a few epochs, to obtain a revised classifier  given as $f_{\theta + \Delta}$. In our experiments, we show that the revised decision function $f_{\hat{\theta}}$ provides improved confidence estimates for AiD and near OOD samples and demonstrate robustness to adversarial attacks, as compared to given classifier $f_{\theta}$.




% \subsection{Discriminator as a Selection Function}
% \label{sec:SC}
% A selection function $g: \mathcal{X} \rightarrow \{0,1\}$ is an addition head on top of a classifier that decides when the classifier should  abstain from making a prediction. We propose to use the discriminator network $D(\mathbf{x})$ as a selection function for $f_{\theta}$. Upon the convergence of the PCE training, the generated samples resemble the in-distribution training data. Far-OOD samples are previously unseen samples which are very different from the training input space. Hence, $D(\cdot)$ can help in detecting such samples.  Our final improved classification function is represented as follow,

% \begin{equation}
%     (f,D)(\mathbf{x})= 
% \begin{cases}
%     f_{\theta + \Delta} (\mathbf{x}),& \text{if } D(\mathbf{x}) \geq h\\
%     \texttt{Abstain},              & \text{otherwise}
% \end{cases}
% \end{equation}

% where, $f_{\theta + \Delta}$ is the fine-tuned classifier and $D(\cdot)$ is a discriminator network from the PCE which serves as a selection function that permits $f$ to make prediction if $D(\mathbf{x})$ exceeds a threshold $h$ and abstain  otherwise.




% %-------------------------------------------------------------------------
% \subsection{Related Work}



% \paragraph{Uncertainty estimation in pre-trained DNN models:} Much of the prior work focused on deriving uncertainty measurements from a pre-trained DNN output~\cite{hendrycks17baseline,temperature_scaling,liang2018enhancing,liu2020energy}, feature representations~\cite{lin2021mood,Lee2018ASU} or gradients~\cite{huang2021on}. Such methods use a threshold-based scoring function to identify OOD samples. The scoring function is derived from softmax confidence scores~\cite{hendrycks17baseline}, scaled logit~\cite{temperature_scaling,lin2021mood}, energy-based scores~\cite{liu2020energy,wang2021can} or gradient-based scores~\cite{huang2021on}. These methods help in identifying OOD samples but did not address the over-confidence problem of DNN, that made identifying OOD non-trivial in the first place~\cite{Hein2019WhyRN,nguyen2015deep}. Our work focuses on mitigating the over-confidence issue by fine-tuning a pre-trained classifier on counterfactually augmented data (CAD). Further, we used the discriminator of the GAN-generator to provide a density score to identify OOD samples. 

% \paragraph{DNN designs for improved uncertainty estimation:} 
% %Designing generalized DNN that provides robust uncertainty estimates has gained significant research attention. 
% The Bayesian neural networks are the gold standard for reliable uncertainty quantification~\cite{neal2012bayesian}. Multiple approximate Bayesian approaches have been proposed to achieve tractable inference and to reduce computational complexity~\cite{NIPS2011_7eb3c8be,Weight_Uncertainty,NIPS2015_bc731692,pmlr-v48-gal16}.  Popular non-Bayesian methods include deep ensembles~\cite{NIPS2017_9ef2ed4b} and their variant~\cite{Snapshot,loss_surface}. However, most of these methods are computationally expensive and requires multiple passes during inference. An alternative approach is to modify DNN training~\cite{label_smoothing_szegedy,zhang2017mixup,manifold_mixup}, loss function~\cite{Mukhoti2020CalibratingDN}, architecture~\cite{sun2021react,Liu2020SimpleAP,Geifman2019SelectiveNetAD} or end-layers~\cite{van2020uncertainty,9156473} to support improved uncertainty estimates in a single forward-pass. Further, methods such as DUQ~\cite{van2020uncertainty} and DDU~\cite{mukhoti2021deterministic} proposed modifications to enable the separation between aleatoric and epistemic uncertainty. Unlike these methods, our approach improves the uncertainty estimates of any existing pre-trained classifier, without changing its architecture or training procedure. We used the discriminative head of the fine-tuned classifier to capture aleatoric uncertainty and the density estimation from the GAN-generator to capture epistemic uncertainty.    

% \paragraph{Uncertainty estimation using GAN:} A popular technique to fix an over-confident classifier is to regularize the model with an auxiliary OOD data which is either realistic~\cite{hendrycks2018deep,Mohseni2020SelfSupervisedLF,PAPADOPOULOS2021138,chen2021atom,LiangEnhancing} or is generated using GAN~\cite{Ren2019LikelihoodRF,lee2018training,Mandal_2019_CVPR,Xiao2020LikelihoodRA,Serr2020Input}. 
% Such regularization helps the classifier to assign lower confidence to anomalous samples, which usually lies in the low-density regions.
% Defining the scope of OOD a-priori is generally hard and can potentially cause a selection bias in the learning. Alternative approaches resort to estimating in-distribution density~\cite{Subramanya2017ConfidenceEI}.
%  Our work fixed the scope of GAN-generation to CAD~\cite{singla2019explanation}. Rather than merging the classifier and the GAN training, we train the GAN in a post-hoc manner to explain the decision of an existing classifier. This strategy defines OOD in the context of pre-trained classifier’s decision boundary. Previously, training with CAD have shown to improved generalization performance on OOD samples~\cite{Kaushik2021ExplainingTE}. However, much of this work is limited to Natural Language Processing, and requires human intervention while curating CAD~\cite{Kaushik2020Learning}. In contrast, we train a GAN-based counterfactual explainer~\cite{singla2021explaining,explaining_in_style} to derive CAD.
 

% %-------------------------------------------------------------------------
% \section{Experiment}

% \newcommand\Tstrut{\rule{0pt}{2.6ex}}         % = `top' strut
% \newcommand\Bstrut{\rule[-1.0ex]{0pt}{0pt}}   % = `bottom' strut
% % \newcommand{\textBF}[1]{%
% %     \pdfliteral direct {2 Tr 0.3 w} %the second factor is the boldness
% %      #1%
% %     \pdfliteral direct {0 Tr 0 w}%
% % }

%   \begin{figure*}[t]
%   \centering
%   \includegraphics[width=1.0\linewidth]{figures/exampleACE.pdf}
%   \footnotesize
%   \caption{ An example of counterfactually generated data by the progressive counterfactual explainer (PCE). More examples are provided in the Supplementary Material.}
%   \label{fig:skin}
% \end{figure*}



% We set up three experiments to compare the baseline model before and after fine-tuning with our proposed counterfactual augmentation:
% First, we assess if the models can correctly capture aleatoric uncertainty by identifying ambiguous test samples. Second, we evaluate the models on OOD detection tasks. We consider a standard OOD task over separate datasets and a challenging task to detect near-OOD samples from previously unseen classes from the same dataset. Finally, we compare the model's behaviour under adversarial attacks.
% %We also visually compare the changes to the loss landscape of the model after fine-tuning. 
% In SM, we show further experiments on more datasets and an ablation study over different components of the PCE. 

%  \emph{Classification tasks: }We consider four classification problems, in increasing level of difficulty: 
%  \begin{enumerate}
%   \item AFHQ~\cite{choi2020afhq}: We consider binary classification over well separated classes, cat vs dog. 
  
     
%     \item Dirty MNIST~\cite{mukhoti2021deterministic}: We consider multi-class classification over hand-written digits 0-6. The dataset is a combination of original MNIST~\cite{lecun1998mnist} and simulated samples from a variational decoder. The samples are generated by combining latent representation of different digits, to simulate ambiguous samples, with multiple plausible labels~\cite{mukhoti2021deterministic}.
    
%     \item CelebA~\cite{liu2015celeba}: We consider a multi-label classification setting over `young' and `smiling' attributes. Without age labels, identifying 'young' faces is a challenging task. 
%     %The dataset is challenging as it comprises several middle-aged people who are arguably neither young nor old, and also has a good class-overlap between `smiling' vs `not-smiling' samples.
    
%     \item Skin lesion (HAM10K)~\cite{tschandl2018ham10000}:  We consider a binary classification to separate Melanocytic nevus (nv) from Melanoma (mel) and Benign Keratosis (bkl) lesions.  Skin lesion classification is a challenging task as different lesions may exhibit similar features~\cite{nachbar1994abcd}. 
   
%  \end{enumerate}




%  \emph{Architecture details: }We consider state-of-the-art DenseNet~\cite{huang2017densely} architecture for the baseline. The \emph{pre-trained} DenseNet model followed the training procedures as described in~\cite{huang2017densely}. In order to keep the architecture and training procedure of PCE simple, we consider the default training parameters from~\cite{abdal2019image2stylegan} for training the StyleGANv2. This encourages reproducibility as we didn't do hyper-parameter tuning for each dataset and classification model. Specifically, we use Adam optimizer to train StyleGANv2 at 256$^2$ resolution for $\sim$200K iterations with a batch size of 8 over 8 GPUs. For training  StyelGANv2, we use a randomly sampled subset $(\sim50\%)$ of the baseline model's training data. For multi-class classification, we consider all pairs of classes while creating counterfactual augmentations. For fine-tuning the baseline, we create a new dataset with 30\% counterfactually generated samples and 70\% real samples from the original training set. All the results are reported on the test set of the baseline. 
 

 
 
%  \emph{Comparison methods: } Our baseline is a standard DNN classifier $f_{\theta}$ trained with cross-entropy loss. For baseline and its post-hoc variant with temperature-scaling (\textbf{TS}), we used threshold over predictive entropy (PE) to identify OOD. PE is defined as $-\sum[f_{\theta}(\mathbf{x})]_k \log[f_{\theta}(\mathbf{x})]_k$. Next, we compared against three methods that changes network training or architecture to learn better uncertainty estimates: \textbf{mixup}: baseline model with mixup training using $\alpha = 0.2$~\cite{zhang2017mixup}, deterministic uncertainty quantification (\textbf{DUQ})~\cite{van2020uncertainty}: baseline model with radial basis function as end-layer and \textbf{DDU}: 
%  a ResNet-18~\cite{he2016deep} model with spectral normalisation and Gaussian Mixture Model (GMM) for density estimation. In DUQ, we use the closest kernel distance to quantify uncertainties. Further, we also compared against two ensemble approaches:  
%  \textbf{MC Dropout} (with 20 dropout samples)~\cite{pmlr-v48-gal16} and five independent runs of baseline as \textbf{5-Ensemble}~\cite{NIPS2017_9ef2ed4b}.   We view the ensemble approaches as an upper bound for uncertainty quantification.  

 
% \begin{table*}[!htb]
% \caption{ \footnotesize Performance of different methods on identifying \textbf{\aid{ambiguous in-distribution (AiD)}} samples. For all metrics, higher is better. The best results from the methods that require a single forward pass at inference time are highlighted.
% %The ensemble approaches form an upper-bound and are for reference only and not comparison.
% %Given a baseline model, our results are averaged over 10 runs of fine-tuning with different augmentation by counterfactual explanation (ACE) datasets. 
% }
% \label{AiD-table}
% \begin{center}
% \footnotesize
% % \resizebox{\textwidth}{!}{%
%     \begin{tabular}{cccccc}
%     \hline
%     \multicolumn{1}{c}{\bf Train }  &  \multicolumn{1}{c}{\bf Method/ }  & \multicolumn{1}{c}{\bf Test-Set} &  \multicolumn{2}{c}{\bf Identifying \aid{AiD}}  \Tstrut{}\\
%     \bf Dataset & \bf Model  & Accuracy & AUC-ROC & TNR@TPR95  \Bstrut{}\\
%     \hline
    
%     & Baseline  &   99.44$\pm$0.02  &  0.87$\pm$0.04  & 48.93$\pm$10 \Tstrut{}\\ 
%      & Baseline+TS~\cite{guo2017temperaturescaling} & 99.45$\pm$0.00  &   0.85$\pm$0.07  &  48.77$\pm$9.8 \\ 
%     & Mixup~\cite{zhang2017mixup} & 99.02$\pm$0.10    & 0.80$\pm$0.05  &  35.66$\pm$6.7 \\ 
%     AFHQ & DUQ~\cite{van2020uncertainty} & 94.00$\pm$1.05  & 0.67$\pm$0.01    & 26.15$\pm$4.5 \\ 
%     & DDU~\cite{mukhoti2021deterministic} & 97.66$\pm$1.10  &  0.74$\pm$0.02  &  19.65$\pm$4.5 \\
%     & \bf Baseline+ACE & \bf 99.52$\pm$0.21  & \bf 0.91$\pm$0.02  &  \bf 50.75$\pm$3.9 \Bstrut{}\\
%     \cline{2-5}
%     & MC Dropout~\cite{pmlr-v48-gal16} & 98.83$\pm$1.12 & 0.87$\pm$0.04 & 51.56$\pm$1.2 \Tstrut{}\\
%     & 5-Ensemble~\cite{NIPS2017_9ef2ed4b} &  99.79$\pm$0.01  &  0.98$\pm$0.01  &  51.93$\pm$2.7 \Bstrut{} \\
%     \hline 
%      & Baseline  &   \bf 95.68$\pm$0.02 & \bf 0.96$\pm$0.00  & 28.5$\pm$2.3 \Tstrut{}\\ 
%      & Baseline+TS~\cite{guo2017temperaturescaling} & \bf 95.74$\pm$0.02 &  0.94$\pm$0.01  & 27.90$\pm$1.3\\ 
%      & Mixup~\cite{zhang2017mixup} & 94.66$\pm$0.16   &  0.94$\pm$0.02  & 25.78$\pm$2.1 \\ 
%     Dirty & DUQ~\cite{van2020uncertainty} & 89.34$\pm$0.44  & 0.67$\pm$0.01   & 23.89$\pm$1.2 \\ 
%     MNIST & DDU~\cite{mukhoti2021deterministic}& 93.52$\pm$1.12   &     0.65$\pm$0.12  &   20.78$\pm$4.0 \\ 
%     & \bf Baseline+ACE &  \bf 95.36$\pm$0.45  &  0.86$\pm$0.01  &  \bf 34.12$\pm$2.6 \Bstrut{}\\
%     \cline{2-5}
%     & MC Dropout~\cite{pmlr-v48-gal16} & 89.50$\pm$1.90  &     0.75$\pm$0.07  &  36.10$\pm$1.8 \Tstrut{}\\ 
%     & 5-Ensemble~\cite{NIPS2017_9ef2ed4b} &  95.90$\pm$0.12   &     0.98$\pm$0.02  &  34.87$\pm$3.4 \Bstrut{}\\
    
%     \hline
    
%     & Baseline  & \bf 89.36$\pm$0.96 & 0.73$\pm$0.01 & 17.18$\pm$1.6 \Tstrut{}\\  
%     & Baseline+TS~\cite{guo2017temperaturescaling} & 89.33$\pm$0.01 & 0.72$\pm$0.02 & 17.21$\pm$1.5   \\  
%     & Mixup~\cite{zhang2017mixup} & 89.04$\pm$0.47 & \bf 0.74$\pm$0.02 & 15.09$\pm$1.9 \\ 
%     CelebA & DUQ~\cite{van2020uncertainty} & 71.75$\pm$0.01 & 0.65$\pm$0.01 & 14.20$\pm$1.0 \\ 
%      & DDU~\cite{mukhoti2021deterministic} & 70.15$\pm$0.02 & 0.67$\pm$0.06 & 11.39$\pm$0.4 \\ 
%      & \bf Baseline+ACE &  86.8$\pm$0.79 & \bf 0.74$\pm$0.06 & \bf 22.36$\pm$ 2.3 \Bstrut{}\\
%     \cline{2-5}
%     & MC Dropout~\cite{pmlr-v48-gal16} & 89.86$\pm$0.33 & 0.73$\pm$0.03 & 19.78$\pm$0.7 \Tstrut{}\\
%     & 5-Ensemble~\cite{NIPS2017_9ef2ed4b} &  90.76$\pm$0.00 & 0.84$\pm$0.11 & 17.79$\pm$0.6 \Bstrut{}\\
%     \hline
    
%      & Baseline  &    85.88$\pm$0.75   & 0.82$\pm$0.06  & 20.52$\pm$3.7 \Tstrut{}\\ 
%      & Baseline+TS~\cite{guo2017temperaturescaling} &  \bf 86.27$\pm$0.40  &     \bf 0.84$\pm$0.03  & 23.34$\pm$2.8 \\ 
%     & Mixup~\cite{zhang2017mixup} &  85.81$\pm$0.61  &  \bf  0.84$\pm$0.04& 31.29$\pm$7.0 \\ 
%     Skin-Lesion & DUQ~\cite{van2020uncertainty} & 75.47$\pm$5.36  &  0.81$\pm$0.02     &  30.12$\pm$4.4\\ 
%     (HAM10K) & DDU~\cite{mukhoti2021deterministic}& 75.84$\pm$2.34   &     0.79$\pm$0.03  &   26.12$\pm$6.6 \\ 
%     & \bf Baseline+ACE & 81.21$\pm$1.12  & \bf 0.84$\pm$0.05  & \bf 71.60$\pm$3.8 \Bstrut{}\\
%     \cline{2-5}
%     & MC Dropout~\cite{pmlr-v48-gal16} & 84.90$\pm$1.17   &  0.85$\pm$0.06  &  43.78$\pm$1.9 \Tstrut{}\\ 
%     & 5-Ensemble~\cite{NIPS2017_9ef2ed4b} &  87.89$\pm$0.13   &     0.86$\pm$0.02  &  40.49$\pm$5.1 \Bstrut{}\\
    
%     \hline
%     \end{tabular}
% \end{center}
% \end{table*}



%  \subsection{Identifying AiD samples}
%  %\emph{Experiment setup:} 
%  %AiD samples have an inherent ambiguity in their class label, arising from the overlapping class definitions. 
%  Curated datasets for image classification are well-defined and provide binarized labels as ground truth. Assigning a label to an image removes ambiguity about its class membership. In the absence of ground truth uncertainty labels, we use the PE estimates from an MC Dropout classifier to label AiD samples. Specifically,   
%  %derive pseudo uncertainty labels for test set. In curated datasets, the test set usually comprises in-distribution (iD) samples with low epistemic uncertainty. Hence, we use PE to quantify aleatoric uncertainty.
%  we sort the test set using PE and consider the top 5 to 10\% samples as AiD. 
 
% In Fig.~\ref{fig:all}, we qualitatively compare the PE distribution from the given baseline and its fine-tuned version (baseline + ACE). Fine-tuning resulted in minor changes to the PE distribution of the iD samples (Fig.~\ref{fig:all}.A). 
%  We observe a significant separation in the PE distribution of AiD samples and the rest of the test set (Fig.~\ref{fig:all}.B), even on the baseline. This suggests that the PE correctly captures the aleatoric uncertainty. Fine-tuning with counterfactual augmentation further enhanced this separation by shifting the PE distribution of AiD samples to the right and assigning a higher PE value to the uncertain samples. 
 
%  The Table~\ref{AiD-table} compares our model to several baselines.  We report the test set accuracy,  the AUC-ROC for the binary task of identifying AiD samples and the  true negative rate (TNR) at 95\% true positive rate (TPR) (TNR@TPR95), which simulates
% an application requirement that the recall of in-distribution
% data should be 95\%~\cite{9156473}. For all metrics higher value is better. Our model outperformed other deterministic models, in identifying AiD samples with a high AUC-ROC and TNR@TPR95 across all datasets. 
% Also, the fine-tuned model retained the predictive accuracy of the baseline in AFHQ and Dirty MNIST datasets. We observe a little drop in test accuracy in  complex classification problems, where multiple classes may look similar, e.g. medical datasets (HAM10K). Fine-tuning makes the decision boundary broader. As a result, the samples near the decision boundary may flip their decision, decreasing accuracy. We consider this drop more like a flag to indicate possible label noise. Please note, in the tables, we highlighted the best results from the methods that require a single forward pass at inference time.


  
  
  

  

% % \fontsize{10pt}{10pt}
% % \selectfont


% \subsection{Detecting OOD samples}

% We consider two tasks to evaluate the model’s OOD detection performance. First, a standard OOD task where OOD samples are derived from a separate dataset. Second, a difficult near-OOD detection task where OOD samples belongs to novel classes from the same dataset, which are not seen during training. We consider the following OOD datasets:
 

%  \begin{enumerate}
 
% \item AFHQ~\cite{choi2020afhq}: We consider ``wild" class from AFHQ to define near-OOD samples. For the far-OOD detection task, we use the CelebA dataset, and also cat/dog images from CIFAR10~\cite{Krizhevsky2009LearningML}.
  
%     \item Dirty MNIST~\cite{mukhoti2021deterministic}: We consider digits 7-9 as near-OOD samples. For far-OOD detection, we use SVHN~\cite{37648} and fashion MNIST~\cite{Xiao2017FashionMNISTAN} datasets.

%  \item CelebA~\cite{liu2015celeba}: We consider images of kids in age-group: 0-11 from the UTKFace~\cite{zhifei2017cvpr} dataset to define the near-OOD samples. For far-OOD detection task, we use the AFHQ and CIFAR10 datasets.
 
%     \item Skin lesion (HAM10K)~\cite{tschandl2018ham10000}: We consider samples from lesion types: Actinic Keratoses and Intraepithelial Carcinoma (akiec), Basal Cell Carcinoma (bcc), Dermatofibroma (df) and Vascular skin lesions (vasc) as near-OOD. For far-OOD, we consider CelebA and an additional simulated dataset with different skin textures/tones.
    
    
    
   
%  \end{enumerate}
 
%  \begin{table*}[!htb]
% \caption{ \footnotesize OOD detection performance for different baselines. \textbf{\nood{Near-OOD}} represents label shift, with samples from the unseen classes of the same dataset. \textbf{\food{Far-OOD}} samples are from a separate dataset.  The numbers are averaged over five runs. 
% %\textcolor{red}{The ensemble approaches form an upper-bound and are for reference only and not comparison.}
% }
% \label{OOD-table}
% \begin{center}
% \scriptsize
% \resizebox{\textwidth}{!}{%
%     \begin{tabular}{cccccccc}
%     \hline 
%     \multicolumn{1}{c}{\bf Train }  &  \multicolumn{1}{c}{\bf Method }  &   \multicolumn{2}{c}{\bf \nood{Near-OOD} (Wild)} &  \multicolumn{2}{c}{\bf \food{Far-OOD} (CIFAR10)} &  \multicolumn{2}{c}{\bf \food{Far-OOD} (CelebA)} \Tstrut{}\\
%     \bf Dataset & \bf   & AUC-ROC & TNR@TPR95 & AUC-ROC & TNR@TPR95 &   AUC-ROC & TNR@TPR95 \Bstrut{}\\
%     \hline
%      & Baseline  &  0.88$\pm$0.04 & 47.40$\pm$5.2    & 0.95$\pm$0.04  & 73.59$\pm$9.4 &   0.95$\pm$0.03 & 70.69$\pm$8.9 \Tstrut{}\\
     
%      & Baseline+TS~\cite{guo2017temperaturescaling} & 0.88$\pm$0.03   & 45.53$\pm$9.8 &   0.95$\pm$0.04  & 71.77$\pm$8.9& 0.95$\pm$0.03 & 65.89$\pm$8.3 \\ 
     
     
%     & Mixup~\cite{zhang2017mixup} & 0.86$\pm$0.06 &  \bf 53.83$\pm$6.8  &  0.82$\pm$0.11  & 57.01$\pm$8.6 & 0.88$\pm$0.13 &70.51$\pm$9.8 \\ 
     
%     AFHQ & DUQ~\cite{van2020uncertainty}       & 0.78$\pm$0.05    & 20.98$\pm$2.0 & 0.67$\pm$0.59  & 16.23$\pm$1.5 & 0.66$\pm$0.55 & 15.34$\pm$2.6  \\ 
     
%      & DDU~\cite{mukhoti2021deterministic} & 0.83$\pm$0.02   & 23.19$\pm$2.6 & 0.90$\pm$0.02    &  32.98$\pm$10& 0.75$\pm$0.02 & 10.32$\pm$5.6 \\ 
    
%     & \bf Baseline+ACE & \bf 0.89$\pm$0.03 &  51.39$\pm$4.4 & \bf 0.98$\pm$0.02    & \bf 88.71$\pm$5.7 &  \bf0.97$\pm$0.03 & \bf 88.87$\pm$9.8 \Bstrut{}\\
    
%      \cline{2-8}
%     & MC-Dropout~\cite{pmlr-v48-gal16} & 0.84$\pm$0.09  & 30.78$\pm$2.9 & 0.94$\pm$0.02  & 73.59$\pm$2.1& 0.95$\pm$0.02 & 71.23$\pm$1.9 \Tstrut{}\\ 
    
    
%     & 5-Ensemble~\cite{NIPS2017_9ef2ed4b} & 0.99$\pm$0.01   & 65.73$\pm$1.2 &   0.97$\pm$0.02  & 89.91$\pm$0.9& 0.99$\pm$0.01 & 92.12$\pm$0.7 \Bstrut{}\\ 
    
    
%     \hline
%      &  \multicolumn{1}{c}{ }  &   \multicolumn{2}{c}{\bf \nood{Near-OOD} (Digits 7-9) } &  \multicolumn{2}{c}{\bf \food{Far-OOD} (SVHN)} &  \multicolumn{2}{c}{\bf \food{Far-OOD} (fMNIST)} \Tstrut{}\\
%      & \bf   & AUC-ROC & TNR@TPR95 & AUC-ROC & TNR@TPR95 &   AUC-ROC & TNR@TPR95 \Bstrut{}\\
%     \cline{3-8}
%     & Baseline  & 0.86$\pm$0.04  &  28.23$\pm$2.9 &  0.75$\pm$0.15 &  51.98$\pm$0.9 & 0.87$\pm$0.02 & 58.12$\pm$1.5 \Tstrut{}\\  
    
%      & Baseline+TS~\cite{guo2017temperaturescaling} & 0.86$\pm$0.01  &  30.12$\pm$2.1 &  0.73$\pm$0.07 &  48.12$\pm$1.5 & 0.89$\pm$0.01 & 61.71$\pm$2.8\\
     
%     Dirty & Mixup~\cite{zhang2017mixup}  & 0.86$\pm$0.02 &  35.46$\pm$1.0 & 0.95$\pm$0.03 &  65.12$\pm$3.1 & 0.94$\pm$0.05 & 66.00$\pm$0.8\\
    
%     MNIST & DUQ~\cite{van2020uncertainty}       &  0.78$\pm$0.01   &  15.26$\pm$3.9 & 0.73$\pm$0.03  & 45.23$\pm$1.9 & 0.75$\pm$0.03 & 50.29$\pm$3.1  \\
    
%      & DDU~\cite{mukhoti2021deterministic} & 0.67$\pm$0.07   &  10.23$\pm$0.9 &   0.68$\pm$0.04  &  39.31$\pm$2.2 & 0.85$\pm$0.02 & 53.76$\pm$3.7 \\ 
     
%      & \bf Baseline+ACE & \bf0.94$\pm$0.02   &   \bf 37.23$\pm$1.9   & \bf 0.98$\pm$0.02  &  \bf 67.88$\pm$3.1 & \bf 0.97$\pm$0.02 & \bf 70.71$\pm$1.1 \Bstrut{}\\
     
     
%     \cline{2-8}
%     & MC-Dropout~\cite{pmlr-v48-gal16} & 0.97$\pm$0.02  &  40.89$\pm$1.5 & 0.95$\pm$0.01 &  62.12$\pm$5.7 & 0.93$\pm$0.02 &65.01$\pm$0.7 \Tstrut{}\\  
    
%     & 5-Ensemble~\cite{NIPS2017_9ef2ed4b} & 0.98$\pm$0.02  &  42.17$\pm$1.0 &  0.82$\pm$0.03&  55.12$\pm$2.1 & 0.94$\pm$0.01 &64.19$\pm$4.2 \Bstrut{}\\ 
    
%     \hline 
%     &  \multicolumn{1}{c}{ }  &   \multicolumn{2}{c}{\bf \nood{Near-OOD} (Kids) } &  \multicolumn{2}{c}{\bf \food{Far-OOD} (AFHQ)} &  \multicolumn{2}{c}{\bf \food{Far-OOD} (CIFAR10)} \Tstrut{}\\
%      & \bf   & AUC-ROC & TNR@TPR95 & AUC-ROC & TNR@TPR95 &   AUC-ROC & TNR@TPR95 \Bstrut{}\\
%      \cline{3-8}
%     & Baseline  & 0.84$\pm$0.02 & 1.25$\pm$0.1 & 0.86$\pm$0.03 & 88.57$\pm$0.9 & 0.79$\pm$0.02 & 29.01$\pm$5.1 \Tstrut{}\\ 
%     & Baseline+TS~\cite{guo2017temperaturescaling} & 0.82$\pm$0.04 & 1.24$\pm$0.1 & 0.87$\pm$0.06 & 88.75$\pm$0.9 & 0.78$\pm$0.04 & 29.01$\pm$5.1  \\ 
%     & Mixup~\cite{zhang2017mixup} & 0.82$\pm$0.08 & 22.18$\pm$2.7 & 0.95$\pm$0.02 & 82.96$\pm$2.5 & 0.79$\pm$0.13 & 30.54$\pm$1.3\\ 
%     CelebA & DUQ~\cite{van2020uncertainty} & 0.80$\pm$0.03 & 14.68$\pm$3.1 & 0.72$\pm$0.07 & 26.62$\pm$7.7 & 0.86$\pm$0.04 & 28.70$\pm$4.1\\ 
%     & DDU~\cite{mukhoti2021deterministic} & 0.73$\pm$0.15  & 7.9$\pm$0.4 & 0.74$\pm$0.13  & 8.18$\pm$0.4 & 0.81$\pm$0.15 & 25.45$\pm$1.4 \\ 
%     & \bf Baseline+ACE & \bf 0.87$\pm$0.03 & \bf 34.37$\pm$2.5 &    \bf 0.96$\pm$0.01 & \bf 96.35$\pm$2.5 & \bf 0.92$\pm$0.05 &  \bf 63.51$\pm$1.5  \Bstrut{}\\
%     \cline{2-8}
%     & MC-Dropout~\cite{pmlr-v48-gal16} & 0.70$\pm$0.10 & 25.62$\pm$1.7 & 0.86$\pm$0.1 & 91.72$\pm$7.5 & 0.74$\pm$0.12 & 64.79$\pm$1.8 \Tstrut{}\\ 
%     & 5-Ensemble~\cite{NIPS2017_9ef2ed4b} & 0.93$\pm$0.03 & 10.35$\pm$0.2 & 0.99$\pm$0.0 & 98.31$\pm$1.2 & 0.92$\pm$0.10 & 61.88$\pm$1.2 \Bstrut{}\\ 
    
%     \hline
%       &  \multicolumn{1}{c}{ }  &   \multicolumn{2}{c}{\bf \nood{Near-OOD} (other lesions) } &  \multicolumn{2}{c}{\bf \food{Far-OOD} (CelebA)} &  \multicolumn{2}{c}{\bf \food{Far-OOD} (Skin-texture)} \Tstrut{}\\
%      & \bf   & AUC-ROC & TNR@TPR95 & AUC-ROC & TNR@TPR95 &   AUC-ROC & TNR@TPR95 \Bstrut{}\\
%     \cline{3-8}
%      & Baseline  &  0.67$\pm$0.04  &8.70$\pm$2.5    &  0.66$\pm$0.06  & 10.00$\pm$3.6 &  0.65$\pm$0.10 & 5.91$\pm$2.8 \Tstrut{}\\ 
     
%       & Baseline+TS~\cite{guo2017temperaturescaling} & 0.67$\pm$0.05   & 8.69$\pm$2.0 & 0.63$\pm$0.06  & 9.24$\pm$4.3 & 0.68$\pm$0.07 & 5.70$\pm$3.2 \\ 
     
%     Skin& Mixup~\cite{zhang2017mixup} & 0.67$\pm$0.01 & 8.52$\pm$2.8   & 0.64$\pm$0.08  & 10.21$\pm$4.0 &  0.72$\pm$0.05 &5.26$\pm$3.1 \\ 
    
%     Lesion & DUQ~\cite{van2020uncertainty} & 0.67$\pm$0.04  &   3.12$\pm$1.8 & 0.89$\pm$0.09 &   11.89$\pm$2.5 & 0.64$\pm$0.03 & 4.8$\pm$1.5\\
    
%      & DDU~\cite{mukhoti2021deterministic} & 0.65$\pm$0.03  &   3.45$\pm$1.9 & 0.75$\pm$0.04 &  15.45$\pm$2.9 & 0.71$\pm$0.05 & 4.19$\pm$1.3 \\
    
%     & \bf Baseline+ACE & \bf0.72$\pm$0.04   & \bf 10.99$\pm$2.8 & \bf 0.97$\pm$0.02   & \bf 66.77$\pm$1.4 &  \bf 0.96$\pm$0.03 & \bf 95.83$\pm$5.0 \Bstrut{} \\
     
%      \cline{2-8}
%     & MC-Dropout~\cite{pmlr-v48-gal16} & 0.67$\pm$0.05   & 9.45$\pm$3.9 &  0.80$\pm$0.07  & 30.00$\pm$3.2&0.56$\pm$0.03  & 10.87$\pm$2.3 \Tstrut{}\\ 
    
    
%     & 5-Ensemble~\cite{NIPS2017_9ef2ed4b} & 0.88$\pm$0.01   & 11.23$\pm$1.7 &  0.91$\pm$0.03  & 27.89$\pm$5.9 & 0.76$\pm$0.02 & 17.89$\pm$3.5 \Bstrut{}\\
    
    
%     \hline
%     \end{tabular}}
% \end{center}
% \end{table*}

  
 
%  %In Fig.~\ref{fig:all}, we qualitatively compare the  distribution over the OOD samples for the given baseline and its improved version (baseline + ACE). 
%  We summarize our qualitative results in Fig.~\ref{fig:all}. We observe much overlap between the predictive entropy (PE) distribution of the near-OOD samples  and in-distribution samples in Fig.~\ref{fig:all}.C. Fine-tuning with counterfactual augmentation helped in reducing this overlap, by amplifying the uncertainty associated with OOD data. Further, in Fig.~\ref{fig:all}.D-E, we observe that the PE distribution from the baseline model does not capture epistemic uncertainty associated with far-OOD samples, but our model successfully disentangles OOD samples from the in-distribution samples by using density estimates from the discriminator of the PCE.
 

%   In Table~\ref{OOD-table}, we report the AUC-ROC and TNR@TPR95 scores on detecting the two types of OOD samples. We first use the discriminator from the PCE to detect far-OOD samples. The discriminator achieved near-perfect AUC-ROC for detecting far-OOD samples. It consistently outperformed the deep ensemble, MC Dropout, and other deterministic methods across all datasets. The near-OOD samples are relatively similar to the training distribution of the discriminator. Hence, the discriminator performed sub-optimally on the near-OOD detection task. We used the PE estimates from the fine-tuned model (baseline + ACE) to detect near-OOD samples. We outperformed all other deterministic methods in identifying near-OOD samples. Overall our model performed better on both near and far-OOD detection tasks with high TNR@TPR95. 
  
   
  
% \subsection{Robustness to Adversarial Attacks}

% \begin{figure}[!htb]
%       \includegraphics[width=1.0\linewidth]{figures/final_attack.pdf}
%     \caption{\footnotesize Plots comparing baseline model before and after fine-tuning (ACE) for different magnitudes of adversarial attack. The figure shows three different attacks -- FGSM~\cite{fgsm_attack}, CW~\cite{carlini_wagner_attack}, DeepFool~\cite{deepfool_attack}, on three different datasets -- HAM10K, AFHQ, MNIST. The x-axis denotes maximum perturbation ($\epsilon$) for FGSM, and iterations in multiples of $10$ for CW and DeepFool. Attack magnitude of $0$ indicates no attack. For CW we used $\kappa=0$ and $5$. (All results are reported on the test-set of the classifier).}\label{fig:adv_attacks}
%   \end{figure}
  
% In this experiment, we compared the baseline model before and after fine-tuning (baseline + ACE) in their robustness to three adversarial attacks: Fast Gradient Sign Method (FGSM)~\cite{fgsm_attack}, Carlini-Wagner (CW)~\cite{carlini_wagner_attack}, and DeepFool~\cite{deepfool_attack}. For each attack setting, we transformed the test set into an adversarial set.  In Fig.~\ref{fig:adv_attacks}, we report the AUC-ROC over the adversarial set as we gradually increase the magnitude of the attack. For FGSM,  we use the maximum perturbation ($\epsilon$) to specify the attack's magnitude. For CW, we gradually increase the number of iterations to an achieve a higher magnitude attack. We set box-constraint parameter as $c=1$, learning rate $\alpha=0.01$ and confidence $\kappa=0,5$. For  DeepFool ($\eta=0.02$), we show results on the best attack. Our improved model (baseline + ACE) consistently out-performed the baseline model in test AUC-ROC, thus showing an improved robustness to all three attacks.  
  
%   % We investigate this further in the supplementary section.


% %-------------------------------------------------------------------------
% \section{Conclusion}

% We propose a novel method to improve the uncertainty quantification of an existing  \emph{pre-trained} DNN by fine-tuning it on counterfactually augmented data. We used a cGAN-based counterfactual explainer to generate the data augmentation. Our fine-tuned model, combined with the discriminator of the GAN, can successfully capture uncertainty over ambiguous samples, unseen near-OOD samples with label shift and far-OOD samples from independent datasets. Comparative post-hoc methods such as thresholding softmax outputs and temperature scaling cannot recover a pre-trained model from over-saturation on log-likelihood loss. Other deterministic methods significantly change the classification model design to enable better uncertainty quantification over OOD samples. These methods require a network to be trained from scratch and are not compatible with a pre-trained classifier. Our proposed strategy reuses the counterfactual explanation model for the given classifier to fix its over-confidence problem. We out-performed state-of-the-art methods for uncertainty quantification on four datasets with varying difficulty levels.
% Furthermore, our improved model also exhibits robustness to prevalent adversarial attacks. We recognize that our proposed strategy involves training a GAN and fine-tuning the classifier with augmented data, which creates a one-time computational overhead. But, once we have a fine-tuned classifier, it requires only a single forward pass, with fast inference. The trained GAN has the added benefit of explaining the given classification model that can help in making it more user-accessible. Our work opens up a new direction for improving uncertainty quantification in existing classification models. We hope our work will contribute to the better adoption of existing models in real-world applications.   

% %-------------------------------------------------------------------------

% {\small
% \bibliographystyle{ieee_fullname}
% \bibliography{egbib}
% }

% \end{document}

